Improving Pre-Trained Multilingual Models with Vocabulary Expansion

Recently, pre-trained language models have achieved remarkable success in a broad range of natural language processing tasks. However, in multilingual setting, it is extremely resource-consuming to pre-train a deep language model over large-scale corpora for each language. Instead of exhaustively pre-training monolingual language models independently, an alternative solution is to pre-train a powerful multilingual deep language model over large-scale corpora in hundreds of languages. However, the vocabulary size for each language in such a model is relatively small, especially for low-resource languages. This limitation inevitably hinders the performance of these multilingual models on tasks such as sequence labeling, wherein in-depth token-level or sentence-level understanding is essential. In this paper, inspired by previous methods designed for monolingual settings, we investigate two approaches (i.e., joint mapping and mixture mapping) based on a pre-trained multilingual model BERT for addressing the out-of-vocabulary (OOV) problem on a variety of tasks, including part-of-speech tagging, named entity recognition, machine translation quality estimation, and machine reading comprehension. Experimental results show that using mixture mapping is more promising. To the best of our knowledge, this is the first work that attempts to address and discuss the OOV issue in multilingual settings.

==> exp_record.tex <==
XNLI dataset:

all use default batch size: 32, epoch:2

translate train:
fr: \\
trn:OOV@token: 0.298995, OOV@subword: 0.000002
test:OOV@token: 0.335622, OOV@subword: 0.001222
el: \\
trn:OOV@token: 0.626950, OOV@subword: 0.000001
test:OOV@token: 0.631486, OOV@subword: 0.000042
bg: \\
trn:OOV@token: 0.555054,OOV@subword: 0.000002
test:OOV@token: 0.595772, OOV@subword: 0.000711
ru: \\
trn: OOV@token: 0.513916, OOV@subword: 0.000002
test: OOV@token: 0.582200, OOV@subword: 0.000966
tr: \\
trn: OOV@token: 0.628085, OOV@subword: 0.000003
test: OOV@token: 0.690172, OOV@subword: 0.000542
vi: \\
trn: OOV@token: 0.182811, OOV@subword: 0.000002
test: OOV@token: 0.199353, OOV@subword: 0.000039
hi: \\
trn: OOV@token: 0.552423, OOV@subword: 0.000002
test:OOV@token: 0.573765, OOV@subword: 0.000081
sw:\\
trn: OOV@token: 0.596112, OOV@subword: 0.000013
test:OOV@token: 0.708371, OOV@subword: 0.000110


translate test:

multi-lingual model: \\
en(train): OOV@token: 0.244768, OOV@subword: 0.000081
fr(test): OOV@token: 0.256168, OOV@subword: 0.000000
ru(test): OOV@token: 0.257748, OOV@subword: 0.000581
tr(test): OOV@token: 0.259787, OOV@subword: 0.000026
vi(test): OOV@token: 0.241748, OOV@subword: 0.000000
th(test): OOV@token: 0.241610, OOV@subword: 0.000000
hi(test): OOV@token: 0.259358, OOV@subword: 0.000000
sw(test): OOV@token: 0.235937, OOV@subword: 0.000000

base&big model: \\
en(train): OOV@token: 0.202453, OOV@subword: 0.000004
en(test): OOV@token: 0.223273, OOV@subword: 0.000000
fr(test): OOV@token: 0.221039, OOV@subword: 0.000000
es(test): OOV@token: 0.218787, OOV@subword: 0.000000
de(test): OOV@token: 0.226032, OOV@subword: 0.000000
el(test): OOV@token: 0.225312, OOV@subword: 0.000000
bg(test): OOV@token: 0.219096, OOV@subword: 0.000000
ru(test): OOV@token: 0.224524, OOV@subword: 0.000000
tr(test): OOV@token: 0.231599, OOV@subword: 0.000027
ar(test): OOV@token: 0.218463, OOV@subword: 0.000006
vi(test): OOV@token: 0.221051, OOV@subword: 0.000000
th(test): OOV@token: 0.214821, OOV@subword: 0.000000
zh(test): OOV@token: 0.221108, OOV@subword: 0.000000
hi(test): OOV@token: 0.236082, OOV@subword: 0.000000
sw(test): OOV@token: 0.218896, OOV@subword: 0.000000
ur(test): OOV@token: 0.235906, OOV@subword: 0.001686






UD dataset:

exp record: tuned parameters on dev and performance on dev:

Jan: has problems in dataset, ignore
pos_v1.2_output_UD_Arabic.b36.e4.0/eval_results.txt:eval_accuracy = 0.5208576584226727
pos_v1.2_output_UD_Basque.b24.e4.0/eval_results.txt:eval_accuracy = 0.9643079477069931
pos_v1.2_output_UD_Bulgarian.b24.e4.0/eval_results.txt:eval_accuracy = 0.9866550803798647
pos_v1.2_output_UD_Croatian.b12.e4.0/eval_results.txt:eval_accuracy = 0.9662036077130417
pos_v1.2_output_UD_Danish.b12.e4.0/eval_results.txt:eval_accuracy = 0.9727427597955707
pos_v1.2_output_UD_Dutch.b24.e4.0/eval_results.txt:eval_accuracy = 0.9754323581703572
pos_v1.2_output_UD_English.b24.e4.0/eval_results.txt:eval_accuracy = 0.9689438523938285
pos_v1.2_output_UD_Estonian.b24.e4.0/eval_results.txt:eval_accuracy = 0.9009433962264151
pos_v1.2_output_UD_Finnish-FTB.b36.e4.0/eval_results.txt:eval_accuracy = 0.8796801624571646
pos_v1.2_output_UD_French.b12.e3.0/eval_results.txt:eval_accuracy = 0.9582382302039179
pos_v1.2_output_UD_German.b48.e4.0/eval_results.txt:eval_accuracy = 0.9486892583120204
pos_v1.2_output_UD_Greek.b12.e4.0/eval_results.txt:eval_accuracy = 0.8069216757741348
pos_v1.2_output_UD_Hindi.b12.e4.0/eval_results.txt:eval_accuracy = 0.8066274810460857
pos_v1.2_output_UD_Hungarian.b12.e4.0/eval_results.txt:eval_accuracy = 0.791407018694654
pos_v1.2_output_UD_Indonesian.b24.e4.0/eval_results.txt:eval_accuracy = 0.9226926736441484
pos_v1.2_output_UD_Irish.b12.e4.0/eval_results.txt:eval_accuracy = 0.8438685208596713
pos_v1.2_output_UD_Italian.b24.e3.0/eval_results.txt:eval_accuracy = 0.9827556623198352
pos_v1.2_output_UD_Japanese-KTC.b12.e2.0/eval_results.txt:eval_accuracy = 0.37899157030491054
pos_v1.2_output_UD_Latin-PROIEL.b24.e4.0/eval_results.txt:eval_accuracy = 0.9698085830682516
pos_v1.2_output_UD_Latin-ITT.b12.e3.0/eval_results.txt:eval_accuracy = 0.9900662251655629
pos_v1.2_output_UD_Latin.b24.e3.0/eval_results.txt:eval_accuracy = 0.911865864144454
pos_v1.2_output_UD_Norwegian.b24.e4.0/eval_results.txt:eval_accuracy = 0.9770477417939507
pos_v1.2_output_UD_Portuguese.b12.e4.0/eval_results.txt:eval_accuracy = 0.9662735361059384
pos_v1.2_output_UD_Polish.b12.e3.0/eval_results.txt:eval_accuracy = 0.9182517787135183
pos_v1.2_output_UD_Persian.b12.e4.0/eval_results.txt:eval_accuracy = 0.9590014462679998
pos_v1.2_output_UD_Swedish.b12.e4.0/eval_results.txt:eval_accuracy = 0.9013983872614065
pos_v1.2_output_UD_Spanish.b48.e4.0/eval_results.txt:eval_accuracy = 0.9593567599761763
pos_v1.2_output_UD_Slovenian.b36.e4.0/eval_results.txt:eval_accuracy = 0.9526424648741174
pos_v1.2_output_UD_Tamil.b12.e4.0/eval_results.txt:eval_accuracy = 0.5399841646872525

dev oov: 
pos_v1.2_output_UD_Arabic:
pos_v1.2_output_UD_Basque:
pos_v1.2_output_UD_Bulgarian:
pos_v1.2_output_UD_Croatian:
pos_v1.2_output_UD_Danish:
pos_v1.2_output_UD_Dutch:
pos_v1.2_output_UD_English:
pos_v1.2_output_UD_Estonian:
pos_v1.2_output_UD_Finnish-FTB:
pos_v1.2_output_UD_French:
pos_v1.2_output_UD_German:
pos_v1.2_output_UD_Greek:
pos_v1.2_output_UD_Hindi:
pos_v1.2_output_UD_Hungarian:
pos_v1.2_output_UD_Indonesian:
pos_v1.2_output_UD_Irish:
pos_v1.2_output_UD_Italian:
pos_v1.2_output_UD_Japanese-KTC:
pos_v1.2_output_UD_Latin-PROIEL:
pos_v1.2_output_UD_Latin-ITT:
pos_v1.2_output_UD_Latin:
pos_v1.2_output_UD_Norwegian:
pos_v1.2_output_UD_Portuguese:
pos_v1.2_output_UD_Polish:
pos_v1.2_output_UD_Persian:
pos_v1.2_output_UD_Swedish:
pos_v1.2_output_UD_Spanish:
pos_v1.2_output_UD_Slovenian:
pos_v1.2_output_UD_Tamil:


test performance:
UD_Arabic.b36.e4/eval_results.txt:eval_accuracy = 0.5334300268855243
test_UD_Basque.b24.e4/eval_results.txt:eval_accuracy = 0.9627471896282924
test_UD_Bulgarian.b24.e4/eval_results.txt:eval_accuracy = 0.9870344476928944
test_UD_Croatian.b12.e4/eval_results.txt:eval_accuracy = 0.9503030303030303
test_UD_Danish.b12.e4/eval_results.txt:eval_accuracy = 0.971617946974847
test_UD_Dutch.b24.e4/eval_results.txt:eval_accuracy = 0.9389435989256938
test_UD_English.b24.e4/eval_results.txt:eval_accuracy = 0.9718680267771757
test_UD_Estonian.b24.e4/eval_results.txt:eval_accuracy = 0.8838912133891214
test_UD_Finnish-FTB.b36.e4/eval_results.txt:eval_accuracy = 0.8772347306119959
test_UD_French.b12.e3/eval_results.txt:eval_accuracy = 0.9517337031900138
test_UD_German.b48.e4/eval_results.txt:eval_accuracy = 0.9357803712886255
test_UD_Greek.b12.e4/eval_results.txt:eval_accuracy = 0.8075158786167961
test_UD_Hindi.b12.e4/eval_results.txt:eval_accuracy = 0.8069714930849563
test_UD_Hungarian.b12.e4/eval_results.txt:eval_accuracy = 0.763302752293578
test_UD_Indonesian.b24.e4/eval_results.txt:eval_accuracy = 0.9237691001697793
test_UD_Irish.b12.e4/eval_results.txt:eval_accuracy = 0.829102329233185
test_UD_Italian.b24.e3/eval_results.txt:eval_accuracy = 0.9821657137981057
test_UD_Japanese-KTC.b12.e2/eval_results.txt:eval_accuracy = 0.38465400061785604
test_UD_Latin.b24.e3/eval_results.txt:eval_accuracy = 0.9470198675496688
test_UD_Latin-ITT.b12.e3/eval_results.txt:eval_accuracy = 0.9934945552255692
test_UD_Latin-PROIEL.b24.e4/eval_results.txt:eval_accuracy = 0.9716221655709111
test_UD_Norwegian.b24.e4/eval_results.txt:eval_accuracy = 0.972497835786109
test_UD_Persian.b12.e4/eval_results.txt:eval_accuracy = 0.95619803945899
test_UD_Polish.b12.e3/eval_results.txt:eval_accuracy = 0.916214335421016
test_UD_Portuguese.b12.e4/eval_results.txt:eval_accuracy = 0.9665928072268621
test_UD_Slovenian.b36.e4/eval_results.txt:eval_accuracy = 0.9502239920358387
test_UD_Spanish.b48.e4/eval_results.txt:eval_accuracy = 0.9603838582677166
test_UD_Swedish.b12.e4/eval_results.txt:eval_accuracy = 0.9122540118761349
test_UD_Tamil.b12.e4/eval_results.txt:eval_accuracy = 0.538964303670186




DuReader:
chinese model: OOV@token: 0.008695, OOV@subword: 0.004005
multilingual model: OOV@token: 0.008661, OOV@subword: 0.003984



RACE:

english model (base and large):
race merged.train: OOV@token: 0.044753, OOV@subword: 0.000000
race middle.test: OOV@token: 0.031460, OOV@subword: 0.000000
race high.test: OOV@token: 0.048599, OOV@subword: 0.000000

multi model: 
race merged.train: OOV@token: 0.077857, OOV@subword: 0.000012
race middle.test: OOV@token: 0.057644 , OOV@subword: 0.000008
race high.test: OOV@token: 0.082922, OOV@subword: 0.000000


WMT18 QE:
en-de
OOV@token: 0.421738, OOV@subword: 0.011963
example:
ar ##zne ##imit ##tel , die sich auf die gast ##roi ##ntes ##tina ##le passage ##zeit aus ##wirken , wie z ##. ##b ##. met ##oc ##lop ##rami ##d , [UNK] die reso ##rp ##tion von pali ##peri ##don bee ##in ##fluss ##en . [SEP] [ ##unk ##] medicinal [ ##unk ##] products [ ##unk ##] affect ##ing [ ##unk ##] gast ##roi ##ntes ##tina ##l [ ##unk ##] transit [ ##unk ##] time [ ##unk ##] medicinal [ ##unk ##] e ##. [ ##unk ##] g ##. [ ##unk ##] met ##oc ##lop ##rami ##de [ ##unk ##] may [ ##unk ##] affect [ ##unk ##] the [ ##unk ##] absorption [ ##unk ##] of [ ##unk ##] pali ##peri ##don ##e [ ##unk ##] . [ ##unk ##] [SEP]

